Endurance-Aware Mapping of Spiking Neural Networks to Neuromorphic Hardware

Neuromorphic computing systems are embracing memristors to implement high density and low power synaptic storage as crossbar arrays in hardware. These systems are energy efficient in executing Spiking Neural Networks (SNNs). We observe that long bitlines and wordlines in a memristive crossbar are a major source of parasitic voltage drops, which create current asymmetry. Through circuit simulations, we show the significant endurance variation that results from this asymmetry. Therefore, if the critical memristors (ones with lower endurance) are overutilized, they may lead to a reduction of the crossbar's lifetime. We propose eSpine, a novel technique to improve lifetime by incorporating the endurance variation within each crossbar in mapping machine learning workloads, ensuring that synapses with higher activation are always implemented on memristors with higher endurance, and vice versa. eSpine works in two steps. First, it uses the Kernighan-Lin Graph Partitioning algorithm to partition a workload into clusters of neurons and synapses, where each cluster can fit in a crossbar. Second, it uses an instance of Particle Swarm Optimization (PSO) to map clusters to tiles, where the placement of synapses of a cluster to memristors of a crossbar is performed by analyzing their activation within the workload. We evaluate eSpine for a state-of-the-art neuromorphic hardware model with phase-change memory (PCM)-based memristors. Using 10 SNN workloads, we demonstrate a significant improvement in the effective lifetime.

==> sections/ev.tex <==
% \subsection{Simulation Setup}
% \label{sec:tech_evaluation}
\subsection{\mr{Use-Case of \tech{}}}\label{sec:scope}
\mr{
Figure~\ref{fig:scope} illustrates the use-case of \tech{} applied for on-line machine learning. We 
use Spike-Timing Dependent Plasticity (STDP)~\cite{dan2004spike}, which is an unsupervised learning algorithm for SNNs, where the synaptic weight between a pre- and a post-synaptic neuron is updated based on the timing of pre-synaptic spikes relative to the post-synaptic spikes.\footnote{Apart from STDP, many other online learning algorithms depend on the activation of both the pre- and post-synaptic neurons.}
STDP is typically used in online settings to improve accuracy of machine learning tasks. 
}

\begin{figure}[h!]
	\centering
	\vspace{-10pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/scope.pdf}}
	\vspace{-10pt}
	\caption{Use-Case of \tech{}.}
	\vspace{-10pt}
	\label{fig:scope}
\end{figure}

\mr{
A machine learning model is first analyzed offline using PyCARL with representative workload and data set. This is to estimate the relative activation frequency of the neurons in the model when it is trained at run-time using current data.
Although neuron activation can deviate at run-time, 
our more detailed analysis shows that using representative workload and data set, such deviations can be limited to only a few neurons in the model.\footnote{\mr{In the worst-case, the lifetime obtained using \tech{} for these few neurons will be similar to \prior{}. However, for most neurons in the model, \tech{} significantly outperforms \prior{}. Therefore, the lifetime obtained using \tech{} is higher (see Section~\ref{sec:lifetime_results}).}}
We have validated this observation for the evaluated applications that use ECG and image data (see Section~\ref{sec:evaluation}).
}

\mr{
The activation information obtained offline is processed using \tech{} (see Figure~\ref{fig:overview} for the details of \tech{}) to generate cluster-to-tile and synapse-to-crossbar mappings. 
The offline trained weight updates are discarded to facilitate relearning of the model from current (in-field) data. The untrained machine learning model is placed onto the hardware using the mappings generated from \tech{}.
}

\mr{
Although online learning is the main focus, \tech{} is also relevant for supervised machine learning, where no weight updates happen at run-time.
By mapping the most active neurons to the farthest corner of a crossbar (i.e., on longest current paths), \tech{} minimizes crossbar temperature, which reduces 1) leakage current and 2) circuit aging.
}

\subsection{Evaluated Applications}
We evaluate 10 SNN-based machine learning applications that are representative of three most commonly-used neural network classes --- convolutional neural network (CNN), multi-layer perceptron (MLP), and recurrent neural network (RNN).
These applications are 
1) LeNet based handwritten digit recognition with \ineq{28 \times 28} images of handwritten digits from the MNIST dataset;
2) AlexNet for ImageNet classification;
3) VGG16, also for ImageNet classification;
4) ECG-based heart-beat classification (HeartClass)~\cite{HeartClassJolpe,das2018heartbeat} using electrocardiogram (ECG) data;
5) {multi-layer perceptron (MLP)-based handwritten digit recognition} (MLP-MNIST)~\cite{Diehl2015} using the MNIST database;
6) {edge detection} (EdgeDet)~\cite{carlsim} on $64 \times 64$ images using difference-of-Gaussian; 
7) {image smoothing} (ImgSmooth)~\cite{carlsim} on $64 \times 64$ images; 
8) {heart-rate estimation} (HeartEstm)~\cite{HeartEstmNN} using ECG data;
9) RNN-based predictive visual pursuit (VisualPursuit)~\cite{Kashyap2018}; and
10) recurrent digit recognition (R-DigitRecog)~\cite{Diehl2015}.
Table~\ref{tab:apps} summarizes the topology, the number of neurons and synapses of these applications, and their baseline accuracy on DYNAP-SE using SpiNeMap~\cite{spinemap}.

% \fixa{
% To demonstrate the potential of \tech{}, we enable STDP-based weight updates~\cite{kheradpisheh2018stdp} in each of these applications.
% %\footnote{Spike-Timing Dependent Plasticity (STDP)~\cite{dan2004spike} is a learning mechanism in SNNs, where the synaptic weight between a pre- and a post-synaptic neuron is updated based on the timing of pre-synaptic inputs relative to the post-synaptic spike.} 
% But our approach is not limited to STDP. 
% }
\vspace{-10pt}
\begin{table}[h!]
	\renewcommand{\arraystretch}{0.8}
	\setlength{\tabcolsep}{2pt}
	\caption{Applications used to evaluate \tech{}.}
	\label{tab:apps}
	\vspace{-10pt}
	\centering
	\begin{threeparttable}
	{\fontsize{6}{10}\selectfont
	    %\vspace{-10pt}
		\begin{tabular}{cc|ccl|c}
			\hline
			\textbf{Class} & \textbf{Applications} & \textbf{Synapses} & \textbf{Neurons} & \textbf{Topology} & \textbf{Accuracy}\\
			\hline
			\multirow{4}{*}{CNN} & LeNet & 282,936 & 20,602 & CNN & 85.1\%\\
			& AlexNet & 38,730,222 & 230,443 & CNN & 90.7\%\\
			& VGG16 & 99,080,704 & 554,059 & CNN & 69.8 \%\\
			& HeartClass~\cite{HeartClassJolpe} & 1,049,249 & 153,730 & CNN & 63.7\%\\
			\hline
			\multirow{3}{*}{MLP} & DigitRecogMLP & 79,400 & 884 & FeedForward (784, 100, 10) & 91.6\%\\
			& EdgeDet \cite{carlsim} & 114,057 &  6,120 & FeedForward (4096, 1024, 1024, 1024) & 100\%\\
			& ImgSmooth \cite{carlsim} & 9,025 & 4,096 & FeedForward (4096, 1024) & 100\%\\
			\hline
 			\multirow{3}{*}{RNN} & HeartEstm \cite{HeartEstmNN} & 66,406 & 166 & Recurrent Reservoir & 100\%\\
 			& VisualPursuit \cite{Kashyap2018} & 163,880 & 205 & Recurrent Reservoir & 47.3\%\\
 			& R-DigitRecog \cite{Diehl2015} & 11,442 & 567 & Recurrent Reservoir & 83.6\%\\
			%Input(32x32x3) - [Conv, Pool]*6 - [Conv, Pool]*6 - FC*84 - FC*10
			\hline
	\end{tabular}}
	%}
% 	\begin{tablenotes}\scriptsize
%         \item[a.] Input(24x24) - [Conv, Pool]*16 - FC*150 - FC*10
%         \item[b.] Input(32x32) - [Conv, Pool]*6 - [Conv, Pool]*16 - Conv*120 - FC*84 - FC*10
%         \item[c.] Input(32x32x3) - [Conv, Pool]*6 - [Conv, Pool]*6 - FC*84 - FC*10
%         \item[d.] Input(82x82) - [Conv, Pool]*16 - [Conv, Pool]*16 - FC*256 - FC*6
%     \end{tablenotes}
	\end{threeparttable}
	%\vspace{12pt}
	\vspace{-10pt}
\end{table}

\subsection{Hardware Models}
We model the DYNAP-SE neuromorphic hardware~\cite{dynapse} with the following configurations.

\begin{itemize}
    \item A tiled array of 4 tiles, each with a 128x128 crossbar. There are 65,536 memristors per crossbar.
    \item Spikes are digitized and communicated between cores through a mesh routing network using the Address Event Representation (AER) protocol.
    \item Each synaptic element is a PCM-based memristor. 
    %In this device, multiple low-resistance states are used for emulating long-term potentiation (LTP; cumulative increase of conductance) and multiple high-resistance states are used for long-term depression (LTD; cumulative and gradual decrease of conductance). Each crossbar uses 1T-$n$R structure, where one access transistor is used to access $n$ OxRAM devices vertically stacked in the back-end of line (BEOL). 
    %Timing parameters are modeled from~\cite{garbin2015hfo}.
\end{itemize}
To test the scalability of \tech{}, we also evaluate DYNAP-SE with 16 and 32 tiles. 

Table \ref{tab:hw_parameters} reports the hardware parameters of DYNAP-SE.

\vspace{-10pt}
\begin{table}[h!]
    \caption{Major simulation parameters extracted from \cite{dynapse}.}
	\label{tab:hw_parameters}
	\vspace{-10pt}
	\centering
	{\fontsize{6}{10}\selectfont
		\begin{tabular}{lp{5cm}}
			\hline
			Neuron technology & 65nm CMOS\\
			\hline
			Synapse technology & PCM\\
			\hline
			Supply voltage & 1.2V\\
			\hline
			Energy per spike & 50pJ at 30Hz spike frequency\\
			\hline
			Energy per routing & 147pJ\\
			\hline
			Switch bandwidth & 1.8G. Events/s\\
			\hline
% 			NVM related & 1T-1R\\
% 			& PCM cell SET: 24 cycles\\
% 			& PCM cell RESET: 18 cycles\\
% 			& Program \& Verify: 35 cycles\\
% 			\hline
	\end{tabular}}
	\vspace{-10pt}
\end{table}

\subsection{Evaluated Techniques}
We evaluate the following techniques (see Fig.~\ref{fig:sota}).
\begin{itemize}
    \item \textbf{\prior{}:} This is the baseline technique to map SNNs to crossbars of a hardware. \prior{} generates clusters from an SNN workload, minimizing the inter-cluster communication. Clusters are mapped to tiles minimizing the energy consumption. Synapses of a cluster are implemented on memristors arbitrarily, without incorporating their endurance.
    \item \textbf{\priorpp{}:} \mr{This is an extension of \prior{}, where the cluster-to-tile mapping is performed using \prior{}, minimizing energy consumption, and the synapse-to-memristor mapping is performed using \tech{}, maximizing effective lifetime.}
    %However, it uses \tech{}'s synapse-to-memristor mapping to implement synapses with higher activation on memristors with higher endurance, and vice versa.
    \item \textbf{\tech{}:} \mr{This is another extension of \prior{}. \tech{} uses only the clustering technique of \prior{}, thereby minimizing the inter-cluster communication, which also improves energy consumption and latency. The cluster-to-tile and synapse-to-memristor mappings are performed using PSO, maximizing the effective lifetime. Furthermore, \tech{} allows to explore the entire Pareto space of energy and lifetime.}
\end{itemize}
\vspace{-10pt}
\begin{figure}[h!]
	\centering
	\centerline{\includegraphics[width=0.5\columnwidth]{images/sota.pdf}}
	\vspace{-10pt}
	\caption{Evaluated techniques.}
	\vspace{-10pt}
	\label{fig:sota}
\end{figure}


\subsection{Evaluated Metric}
We evaluate the following metrics.
\begin{itemize}
    \item \textbf{Effective lifetime:} This is the minimum effective lifetime of all memristors in the hardware.
    \item \textbf{Energy consumption:} This is the total energy consumed on the hardware. We also evaluate the static and dynamic energy consumption.
    \item \textbf{Compilation time:} This is the time it takes for the PSO to find a solution.
\end{itemize}

==> sections/evaluation.bk.tex <==
% \subsection{Simulation Setup}
% \label{sec:tech_evaluation}

\subsection{Evaluated Applications}
We evaluate 10 SNN-based machine learning applications that are representative of three most commonly-used neural network classes --- convolutional neural network (CNN), multi-layer perceptron (MLP), and recurrent neural network (RNN).
These applications are 
1) LeNet~\cite{lenet} based handwritten digit recognition with \ineq{28 \times 28} images of handwritten digits from the MNIST dataset \cite{deng2012mnist};
2) AlexNet~\cite{alexnet} for ImageNet classification~\cite{deng2009imagenet};
3) VGG16~\cite{vgg16}, also for ImageNet classification~\cite{deng2009imagenet};
4) ECG-based heart-beat classification (HeartClass)~\cite{HeartClassJolpe} using electrocardiogram (ECG) data from the PhysioNet database~\cite{moody2001physionet};
5) {multi-layer perceptron (MLP)-based handwritten digit recognition} (MLP-MNIST)~\cite{Diehl2015} using the MNIST database;
6) {edge detection} (EdgeDet)~\cite{carlsim} on $64 \times 64$ images using difference-of-Gaussian; 
7) {image smoothing} (ImgSmooth)~\cite{carlsim} on $64 \times 64$ images; 
8) {heart-rate estimation} (HeartEstm)~\cite{HeartEstmNN} using ECG data;
9) RNN-based predictive visual pursuit (VisualPursuit)~\cite{Kashyap2018}; and
10) recurrent digit recognition (R-DigitRecog)~\cite{Diehl2015}.
Table~\ref{tab:apps} summarizes the topology, the number of neurons and synapses of these applications, and their baseline accuracy on DYNAP-SE using SpiNeMap~\cite{spinemap}.

\fixa{
To demonstrate the potential of \tech{}, we enable STDP-based weight updates~\cite{kheradpisheh2018stdp} in each of these applications.\footnote{Spike-Timing Dependent Plasticity (STDP)~\cite{dan2004spike} is a learning mechanism in SNNs, where the synaptic weight between a pre- and a post-synaptic neuron is updated based on the timing of pre-synaptic inputs relative to the post-synaptic spike.} But our approach is not limited to STDP. 
}

\begin{table}[h!]
	\renewcommand{\arraystretch}{0.8}
	\setlength{\tabcolsep}{2pt}
	\caption{Applications used to evaluate \tech{}.}
	\label{tab:apps}
	\vspace{-5pt}
	\centering
	\begin{threeparttable}
	{\fontsize{6}{10}\selectfont
	    %\vspace{-10pt}
		\begin{tabular}{cc|ccl|c}
			\hline
			\textbf{Class} & \textbf{Applications} & \textbf{Synapses} & \textbf{Neurons} & \textbf{Topology} & \textbf{Accuracy}\\
			\hline
			\multirow{4}{*}{CNN} & LeNet~\cite{lenet} & 282,936 & 20,602 & CNN & 85.1\%\\
			& AlexNet~\cite{alexnet} & 38,730,222 & 230,443 & CNN & 90.7\%\\
			& VGG16~\cite{vgg16} & 99,080,704 & 554,059 & CNN & 69.8 \%\\
			& HeartClass~\cite{HeartClassJolpe} & 1,049,249 & 153,730 & CNN & 63.7\%\\
			\hline
			\multirow{3}{*}{MLP} & DigitRecogMLP & 79,400 & 884 & FeedForward (784, 100, 10) & 91.6\%\\
			& EdgeDet \cite{carlsim} & 114,057 &  6,120 & FeedForward (4096, 1024, 1024, 1024) & 100\%\\
			& ImgSmooth \cite{carlsim} & 9,025 & 4,096 & FeedForward (4096, 1024) & 100\%\\
			\hline
 			\multirow{3}{*}{RNN} & HeartEstm \cite{HeartEstmNN} & 66,406 & 166 & Recurrent Reservoir & 100\%\\
 			& VisualPursuit \cite{Kashyap2018} & 163,880 & 205 & Recurrent Reservoir & 47.3\%\\
 			& R-DigitRecog \cite{Diehl2015} & 11,442 & 567 & Recurrent Reservoir & 83.6\%\\
			%Input(32x32x3) - [Conv, Pool]*6 - [Conv, Pool]*6 - FC*84 - FC*10
			\hline
	\end{tabular}}
	%}
% 	\begin{tablenotes}\scriptsize
%         \item[a.] Input(24x24) - [Conv, Pool]*16 - FC*150 - FC*10
%         \item[b.] Input(32x32) - [Conv, Pool]*6 - [Conv, Pool]*16 - Conv*120 - FC*84 - FC*10
%         \item[c.] Input(32x32x3) - [Conv, Pool]*6 - [Conv, Pool]*6 - FC*84 - FC*10
%         \item[d.] Input(82x82) - [Conv, Pool]*16 - [Conv, Pool]*16 - FC*256 - FC*6
%     \end{tablenotes}
	\end{threeparttable}
	%\vspace{12pt}
	\vspace{-10pt}
\end{table}

\subsection{Hardware Models}
We model the DYNAP-SE neuromorphic hardware~\cite{dynapse} with the following configurations.

\begin{itemize}
    \item A tiled array of 4 tiles, each with a 128x128 crossbar. There are 65,536 memristors per crossbar.
    \item Spikes are digitized and communicated between cores through a mesh routing network using the Address Event Representation (AER) protocol.
    \item Each synaptic element is a PCM-based memristor. 
    %In this device, multiple low-resistance states are used for emulating long-term potentiation (LTP; cumulative increase of conductance) and multiple high-resistance states are used for long-term depression (LTD; cumulative and gradual decrease of conductance). Each crossbar uses 1T-$n$R structure, where one access transistor is used to access $n$ OxRAM devices vertically stacked in the back-end of line (BEOL). 
    %Timing parameters are modeled from~\cite{garbin2015hfo}.
\end{itemize}
To test the scalability of \tech{}, we also evaluate DYNAP-SE with 16 and 32 tiles. 

Table \ref{tab:hw_parameters} reports the hardware parameters of DYNAP-SE.

\begin{table}[h!]
    \caption{Major simulation parameters extracted from \cite{dynapse}.}
	\label{tab:hw_parameters}
	\vspace{-10pt}
	\centering
	{\fontsize{6}{10}\selectfont
		\begin{tabular}{lp{5cm}}
			\hline
			Neuron technology & 65nm CMOS\\
			\hline
			Synapse technology & PCM\\
			\hline
			Supply voltage & 1.2V\\
			\hline
			Energy per spike & 50pJ at 30Hz spike frequency\\
			\hline
			Energy per routing & 147pJ\\
			\hline
			Switch bandwidth & 1.8G. Events/s\\
			\hline
% 			NVM related & 1T-1R\\
% 			& PCM cell SET: 24 cycles\\
% 			& PCM cell RESET: 18 cycles\\
% 			& Program \& Verify: 35 cycles\\
% 			\hline
	\end{tabular}}
	\vspace{-10pt}
\end{table}

\subsection{Evaluated Techniques}
We evaluate the following techniques (see Fig.~\ref{fig:sota}).
\begin{itemize}
    \item \textbf{\prior{}:} This is the baseline technique to map SNNs to crossbars of a hardware. \prior{} generates clusters from an SNN workload, minimizing the inter-cluster communication. Clusters are mapped to tiles minimizing the energy consumption on the shared interconnect. Synapses of a cluster are implemented on memristors arbitrarily, without incorporating their endurance.
    \item \textbf{\priorpp{}:} This is a modified version of \prior{}, where the cluster-to-tile mapping is performed using \prior{}. However, it uses \tech{}'s synapse-to-memristor mapping to implement synapses with higher activation on memristors with higher endurance, and vice versa.
    \item \textbf{\tech{}:} This is the proposed endurance-oriented technique to map SNN workloads to neuromorphic hardware. \tech{} uses the clustering technique of \prior{}, thereby minimizing the inter-cluster communication, which also improves energy consumption and latency. However, the proposed cluster-to-tile mapping is performed using PSO to maximize the effective lifetime. Synapses of a cluster are implemented on memristors of a crossbar using the proposed synapse-to-memristor mapping.
\end{itemize}
\vspace{-10pt}
\begin{figure}[h!]
	\centering
	\centerline{\includegraphics[width=0.6\columnwidth]{images/sota.pdf}}
	\vspace{-10pt}
	\caption{Evaluated techniques.}
	\label{fig:sota}
\end{figure}


\subsection{Evaluated Metric}
We evaluate the following metrics.
\begin{itemize}
    \item \textbf{Effective lifetime:} This is the minimum effective lifetime of all memristors in the hardware.
    \item \textbf{Energy consumption:} This is the total energy consumed on the hardware. We also evaluate the static and dynamic energy consumption.
    \item \textbf{Compilation time:} This is the time it takes for the PSO to find a solution.
\end{itemize}

==> sections/extra.tex <==
is used, which is a function of temperature of the PCM cell. To evaluate the endurance we need to determine the temperature of the PCM cell. Fig.~\ref{fig:Model block} presents the process of calculating the temperature of the PCM cell. First the crystalline fraction is computed from the inputs and results from the previous state. We assume that initially the PCM cell temperature is equal to the ambient temperature. This Crystalline Fraction is re-input to thermal conductivity module and PCMR module that calculates the thermal conductivity and resistance of the PCM cell corresponding to the crystalline fraction. The changed conductivity exerts an impact on heat dissipation whereas the resistance of the PCM cell changes the joule heating. Finally the temperature of the PCM cell is computed which is based on joule heating and heat dissipation. This temperature is fed back to the crystalline fraction module for next iteration. 
\begin{figure}[h!]
	\centering
	\centerline{\includegraphics[width=0.99\columnwidth]{images/flowchart.pdf}}
	\caption{Model Block Diagram.}
		\label{fig:Model block}
\end{figure}


\textbf{A. Crystalline Fraction Module, $V_C$}\\
Crystalline fraction presents the transformation of solid from one state to another as a function of time and temperature. Johnson-Mehl-Avrami developed a mathematical expression that describes this transformation of solid based on nucleation ~\cite{Avrami1941}, ~\cite{Wei2006}. According to JMA equation,
\begin{equation}
V_C=exp\left[-\alpha \times\frac{(T_{PCM}-T_{amb})}{T_m}\times t\right]
\end{equation}
where $T_{PCM}$ is the temperature of PCM cell, $T_{amb}$ is the ambient temperature and $t$ is the programming time. $\alpha$ and $T_m$ are fitting parameters.When $V_C=1$ the cell is in crystalline state. As the cell temperature increases, $V_C$ approaches to zero and the cell transforms to amorphous state. If the cell temperature $T_{PCM}$ is beyond the melting temperature the crystalline fraction is set to zero.\par
\vspace{5mm}
\textbf{B. Thermal Conductivity Module, $k$}\\
Thermal conductivity decreases with temperature and changes with phase transition~\cite{Lyeo2006}. This relationship gives the following expression of thermal conductivity~\cite{Liao2008},
\begin{equation}
\label{eq:k}
k=(k_a-k_c)\times V_C+k_a
\end{equation}
where $k_a=0.002 WK^{-1}cm^{-1}$ for amorphous GST,  $k_c=0.005 WK^{-1}cm^{-1}$ for crystalline GST. When $T_{PCM}$ reaches the melting temperature,$V_C$ turns out to be zero and thermal conductivity decreases to $k_a$.\par
\vspace{5mm}
\textbf{C. PCMR Module, $R_{PCM}$}\\
The effective resistance of PCM cell is modeled as a function of temperature and crystalline fraction. For simplification we assume that the effective resistance, $R_{PCM}$ varies between set resistance, $R_{set}(10k\Omega)$ and reset resistance, $R_{reset}(200k\Omega)$. 
\begin{equation}
\label{eq:RPCM}
R_{PCM}=R_{set}+(1-V_C)\times(R_{reset}-R{set})
\end{equation}
At ambient temperature the PCM cell is completely crystallized. This results in $V_C=1$ and $R_{PCM}=R_{set}$.\par
\vspace{5mm}
\textbf{D. Heat and Temperature Calculation Module}\\
The temperature of the PCM cell is computed using Joule heating, $W_j$ and heat dissipation, $W_d$ which is given by the following equation ~\cite{Liao2008},
\begin{equation}
\label{eq:TPCM}
T_{PCM}=\int \frac{W_j-W_d}{C\times V}dt
\end{equation}
where C and V are heat capacity of GST and volume of the active region of the cell respectively. The heat generation in the PCM cell is given by,
\begin{equation}
\label{eq:joule heating}
W_j=I_{PCM}^2\times R_{PCM}
\end{equation}
where $I_{PCM}$ is the current through the PCM cell and $R_{PCM}$ is the effective resistance of the cell calculated using equation~\ref{eq:RPCM}. Part of this generated heat is dissipated to the surrounding and this heat dissipation is given by the equation~\cite{Liao2007},
\begin{equation}
\label{eq:heat dissipation}
W_d=-k\sum\Delta T
\end{equation}
where $\Delta T$ represents the temperature dispersion around the active region and expressed as, 
\begin{equation}
\label{eq:delta_T}
    \Delta T=\frac{\partial T_{PCM}}{\partial x}+\frac{\partial T_{PCM}}{\partial y}+ \frac{\partial T_{PCM}}{\partial z}
\end{equation}
For simplicity we assume that the heat is mainly dispersed along the thickness of the cell and the temperature outside the dispersion region is close to ambient temperature. These assumptions yield to one dimensional equation.Thus equation~\ref{eq:heat dissipation} can be written as~\cite{Kwong2008},~\cite{Wei2012},
\begin{equation}
\label{eq:Wd}
    W_d=\frac{kV}{l^2}(T_{PCM}-T_{amb})
\end{equation}
where $l$ is the thickness of the GST material and thermal conductivity, $k$ is computed using equation~\ref{eq:k}. Substitution of equation~\ref{eq:joule heating} and ~\ref{eq:Wd} in equation ~\ref{eq:TPCM} yields,
\begin{equation}
    \frac{dT_{PCM}}{dt}=\frac{W_j-W_d}{C\times V}
\end{equation}
Solving this ODE gives,
\begin{equation}
    T_{PCM}=\frac{I_{PCM}^2R_{PCM}l^2}{kV}-C_1 exp\left(-\frac{kt}{l^2C}\right)+T_{amb}
\end{equation}
Initially the PCM cell is assumed to be in ambient temperature. This boundary condition is used to determine the constant $C_1$. Finally the cell temperature is modeled as, 
\begin{equation}
\label{eq:final TPCM}
    T_{PCM}=\frac{I_{PCM}^2R_{PCM}l^2}{kV}-\left[1-exp\left(-\frac{kt}{l^2C}\right)\right]+T_{amb}
\end{equation}
As we consider set to reset operation equation~\ref{eq:final TPCM} can be normalized to avoid the complexity of calculation which is formulated as,
\begin{equation}
\label{eq:normalized TPCM}
    T_{PCM}=\left(\frac{\beta I_{reset}^2R_{PCM}}{k}\right)+T_{amb}
    \end{equation}
where $\beta$ is the fitting parameter and $I_{reset}$ is the RESET programming current.\par
